Anticipating Information Needs Based on Check-in Activity

In this work we address the development of a smart personal assistant that is capable of anticipating a user's information needs based on a novel type of context: the person's activity inferred from her check-in records on a location-based social network. Our main contribution is a method that translates a check-in activity into an information need, which is in turn addressed with an appropriate information card. This task is challenging because of the large number of possible activities and related information needs, which need to be addressed in a mobile dashboard that is limited in size. Our approach considers each possible activity that might follow after the last (and already finished) activity, and selects the top information cards such that they maximize the likelihood of satisfying the user's information needs for all possible future scenarios. The proposed models also incorporate knowledge about the temporal dynamics of information needs. Using a combination of historical check-in data and manual assessments collected via crowdsourcing, we show experimentally the effectiveness of our approach.

==> wsdm2017-activity-07.tex <==
\section{Evaluation}
\label{sec:evaluation}

The closest approximation of just-in-time information consumption in the real mobile settings is usage of specialized applications installed on a device. The selection of applications that people use is relatively wide and in \todo{X\%} users prefer them over seeking for the same kind of information using a search engine \todo{[citation]}.

In our evaluation methodology we use this fact and we employ an application usage log from mobile devices collected in  the Lausanne Data Collection Campaign (LDCC)~\cite{laurila:2012:mdc}. Apart from various sensory data, it contains information about application usage and users' location in form of semantic labels collected over a year-long period from $185$ individuals. We map the labels to corresponding top-level activities and the applications to information needs as described in Section~\ref{sec:evaluation:preproc}.

\subsection{Evaluation Dataset Preprocessing}
\label{sec:evaluation:preproc}

The Lausanne Data Collection Campaign (LDCC) was an effort to collect longitudinal data from Nokia smartphones that was initiated in 2009. The dataset was divided into parts according to $3$ predefined prediction tasks: a) Semantic place prediction, b) Next place prediction and c) Demographic attribute prediction. In order to generate data for the first task, the participants were asked to label their most and least frequently visited places with one of the following $10$ semantic labels:

\begin{itemize}
	\item Home
	\item Home of a friend
	\item My workplace/school
	\item Location related to transportation
	\item Workplace/school of a friend
	\item Place for outdoor sports
	\item Place for indoor sorts
	\item Restaurant or bar
	\item Shop or shopping center
	\item Holiday resort
\end{itemize}

Due to privacy concerns, the exact locations were not provided, however 493 locations were assigned one of the above labels and locations where users stayed at least $10$ minutes were extracted into \texttt{visit\_sequence\_10min} dataset. Additional context was logged including the following data:
 

\begin{description}
	\item [Demographic] attributes such as participant's age, gender and employment status.
	\item [Calendar] indicating participant's planned events and whether she is busy.
	\item [GSM and Bluetooth] data revealing information about number of nearby devices.
	\item [Accelerometer] measurements indicating the type of participant's movement activity (e.g., walking, traveling by bus or car, being stationary).
	\item [Call logs] recording time and duration of voice and message communication.
	\item [System variables] indicating state of the mobile phone such as battery percentage, charging status or amount of available RAM.
\end{description}




\subsection{Ground Truth}
\label{sec:evaluation:gt}
The ground truth for the RQ1, i.e., finding the common information needs with respect to an activity, is acquired by finding applications used while the user is visiting locations with a corresponding semantic label. Since these labels are linked to the activities from our experiments, the most frequent applications within a certain label indicate the most sought for information needs during an activity. 

In similar fashion we extract the most common applications used before, during and after visiting a location with a certain label to establish a ground truth for the RQ2, i.e., to answer how information needs change throughout an activity.

The ground truth for the RQ3, i.e., how are information needs influenced by the previous activity, is based on applications used during a session of location visits. These sessions, equally to the experimental settings, are series of visited POIs where two consecutive check-ins don't exceed period of $6$ hours. The ground truth is then composed of applications used within a location with certain label given a preceding location label.

\subsection{Baseline}
\label{sec:evaluation:baseline}
We use extracted query suggestions ranked according to their frequency as described in Section~\ref{sec:expsetup} as our baseline.  \todo{Explain this baseline selection.}

\subsection{Evaluation Metrics}
\label{sec:evaluation:metrics}

\subsubsection*{Information needs ranking}
\label{sec:evaluation:ranking}
In our crowdsourcing experiments, we introduced $3$ different approaches of data collection: (1) Free text input of information needs, (2) `dropdown selection' from a predefined set of needs and (3) card-based selection. In order to evaluate our predictions against the ground truth, we apply different evaluation metrics:

\begin{itemize}
\item Precision - binary
	\item Recall - binary (only for the free text)
	\item NDCG 
 		\begin{itemize}
			\item 3+ people $\rightarrow$ score: 3, 
			\item 2 people $\rightarrow$ score: 2, 
			\item 1 person $\rightarrow$ score: 1
		\end{itemize}
\end{itemize}

\subsubsection*{Context: Time around the activity}
\label{sec:evaluation:time}
\todo{Describe evaluation of pre/during/after activity IN}.


\subsubsection*{Context: Previous activity}
\label{sec:evaluation:prevact}
\todo{Describe evaluation of IN given the previous activity}.

\subsubsection*{Anticipation of next information needs}
\label{sec:evaluation:anticip}
\todo{Describe evaluation of anticipation of next IN given the current activity}.

